Steering Vectors are an Adversarial Attack Surface

Activation steering has become a popular way to control Large Language Model (LLM) behavior without fine-tuning. Since the technique is plug-and-play, users share datasets and precomputed vectors to steer model activations. However, we show that a \emph{stealth data poisoning attack} silently compromises this pipeline. By substituting $4{-}6\%$ of tokens in the steering dataset, an attacker can silently align the resulting vector with an anti-refusal direction. This jailbreaks the target model while preserving the intended steering effect on benign prompts. Under this threat model, a malicious actor can distribute an apparently safe bundle containing texts, vectors, and weights, alongside an equivalence certificate that the end-user can verify. We test the attack on two open-weight model families and eight model-attribute combinations, observing that poisoned vectors reach an absolute attack success rate (ASR) of $20{-}55\%$, $+19\%$ to $+51\%$ over a clean reference. Finally, we find that a refusal-direction orthogonalization defense can recover ${\approx}82\%$ of the ASR gap without harming benign behavior.

==> sections/5_discussion.tex <==

\paragraph{Possible defenses.}
Several mitigations are worth investigating beyond the orthogonalisation defense of \Cref{sec:defense_ortho}:
(i) screening the computed steering vector for suspicious cosine with known dangerous directions (e.g., $\mathbf{r}$): a registry plus a low threshold is the most direct detector;
(ii) auditing dataset entries for elevated perplexity relative to reference texts, though our attack keeps modified-text PPL under a hard cap;
(iii) computing steering vectors from multiple independent datasets and checking for directional consistency, on the assumption that an attacker cannot poison every upstream source;
(iv) requiring provenance tracking and cryptographic signing of datasets.
Benign-prompt behavioural checks alone are insufficient since the poisoned vector passes them by construction, and an adaptive attacker aware of (i) can co-optimise under a cap on $\cos(\mathbf{v},\mathbf{r})$ to stay below the defender's threshold; quantifying how much lift survives such a constraint is left to future work.

\paragraph{Broader implications.}
The entangled nature of LLM representations means any post-hoc intervention in activation space carries dual-use risk: a vector computed for one purpose can silently encode another while continuing to perform the first.
As activation steering matures from a research tool into a deployment practice, integrity verification mechanisms will be essential, and they will need to test the artefact on \emph{adversarial} inputs to detect attacks of this kind.


==> sections/7_theory.tex <==
The poisoning objective in \Cref{eq:objective} is a discrete, nonconvex
optimization problem over token sequences. We therefore do not claim that
Algorithm~\ref{alg:stealth_attack} finds a globally optimal poisoned dataset.
Instead, we establish algorithmic guarantees showing that the procedure remains
inside the stealth-preserving feasible set, monotonically improves the attack
objective whenever it accepts an update, and admits a local-optimality
interpretation for an exhaustive variant. Full formal statements and proofs are
given in \Cref{app:theoretical_guarantees}.

\begin{theorem}[Informal: feasibility, monotonicity, and termination]
\label{thm:informal_monotonicity}
Let $\mathcal D$ be the set of poisoned datasets satisfying the attack
constraints: at most $n_{\mathrm{mod}}$ edits per text, replacements restricted
to the safe vocabulary and precomputed neighbor table, protected suffix tokens
fixed, and perplexity at most $\tau$ for every modified text. For any feasible
dataset $D \in \mathcal D$, let
\[
    F(D) = \cos(\mathbf v(D), \mathbf r),
\]
where $\mathbf v(D)$ is the steering vector induced by $D$.

Algorithm~\ref{alg:stealth_attack} maintains $D_t \in \mathcal D$ at every
iteration. Moreover, along the sequence of datasets
$D_0,D_1,\ldots$ produced by the algorithm,
\[
    F(D_{t+1}) \geq F(D_t)
\]
for every iteration $t$, with strict inequality whenever an update is accepted.
Consequently, the final poisoned dataset $D_T$ satisfies
\[
    F(D_T) \geq F(D_0).
\]
Since the feasible set is finite, the algorithm can make only finitely many
strict improvements; together with the iteration budget $B$ and patience
parameter $P$, this gives finite termination.
\end{theorem}

This theorem formalizes the basic correctness property of the attack. Candidate
generation only proposes replacements from the safe neighbor table, skips edits
that would exceed the per-text budget, and excludes protected suffix tokens.
Candidate evaluation rejects texts that violate the perplexity cap. Therefore
every accepted update remains feasible. The monotonicity statement follows from
the acceptance rule: rejected candidates leave the dataset unchanged, while
accepted candidates must strictly improve the cosine alignment with
$\mathbf r$.

\begin{theorem}[Informal: coordinatewise local optimality of exhaustive search]
\label{thm:informal_local_optimality}
Consider an idealized exhaustive variant of Algorithm~\ref{alg:stealth_attack}
that, whenever a text is selected, evaluates every feasible modification of that
text rather than sampling $C$ candidates. If this exhaustive variant completes a
full sweep over all $2N$ positive and negative texts without accepting an
update, then the returned dataset is coordinatewise locally optimal: no feasible
single-text modification can further increase
\[
    F(D) = \cos(\mathbf v(D), \mathbf r).
\]
\end{theorem}

This result clarifies what the practical sampled algorithm approximates. The
implementation used in our experiments evaluates only a random batch of
candidates for computational efficiency, so failing to find an improvement does
not imply that no improvement exists. In contrast, the exhaustive variant checks
the entire feasible neighborhood induced by modifying one text at a time. A full
non-improving sweep therefore certifies local optimality with respect to those
coordinate moves.

\begin{theorem}[Informal: bounded steering-vector perturbation]
\label{thm:informal_perturbation}
Assume the hidden-state map $x \mapsto \mathbf h_\ell(x)$ is $L$-Lipschitz with
respect to perturbations of the input token embeddings. Also assume that every
allowed neighbor replacement satisfies
\[
    \|\mathbf e_t - \mathbf e_{t'}\|_2 \leq \rho .
\]
Then any feasible poisoned dataset $\tilde D$ satisfies
\[
    \|\mathbf v(\tilde D) - \mathbf v(D_0)\|_2
    \leq
    2 L n_{\mathrm{mod}} \rho .
\]
\end{theorem}

The perturbation bound connects the discrete stealth constraints to movement in
activation space. Each text changes in at most $n_{\mathrm{mod}}$ token
positions, and each allowed replacement moves the corresponding embedding by at
most $\rho$. Under the Lipschitz assumption, this bounds the hidden-state change
for each text. Since the steering vector is the difference between the mean
positive and mean negative hidden states, the total deviation is bounded by the
sum of the positive-side and negative-side perturbations.

Together, these results should be interpreted as algorithmic guarantees rather
than global optimization guarantees. They show that
Algorithm~\ref{alg:stealth_attack} is a feasible monotone ascent procedure over a
finite constrained search space, and that its sampled search can be viewed as a
tractable stochastic approximation to exhaustive coordinate ascent.
